DB-GPT-Hub: Towards Open Benchmarking Text-to-SQL Empowered by Large Language Models

Large language models (LLMs) becomes the dominant paradigm for the challenging task of text-to-SQL. LLM-empowered text-to-SQL methods are typically categorized into prompting-based and tuning approaches. Compared to prompting-based methods, benchmarking fine-tuned LLMs for text-to-SQL is important yet under-explored, partially attributed to the prohibitively high computational cost. In this paper, we present DB-GPT-Hub, an open benchmark suite for LLM-empowered text-to-SQL, which primarily focuses on tuning LLMs at large scales. The proposed benchmark consists of: 1. a standardized and comprehensive evaluation of text-to-SQL tasks by fine-tuning medium to large-sized open LLMs; 2. a modularized and easy-to-extend codebase with mainstream LLMs and experimental scenarios supported, which prioritizes fine-tuning methods but can be easily extended to prompt-based setting. Our work investigates the potential gains and the performance boundaries of tuning approaches, compared to prompting approaches and explores optimal solutions tailored to specific scenarios. We hope DB-GPT-Hub, along with these findings, enables further research and broad applications that would otherwise be difficult owing to the absence of a dedicated open benchmark. The project code has been released at https://github.com/eosphoros-ai/DB-GPT-Hub.

==> latex/experiment_old.tex <==
To demonstrate the utility of our DB-GPT-Hub in providing fair, comprehensive, and rigorous comparisons among text-to-SQL methods, we conduct extensive experiments and present some main results in terms of generalization and efficiency under various datasets and scenarios. The complete
experimental results are presented in  due to the space limitation.

\subsection{Result and Analysis}


% \paragraph{Dataset.} We evaluate Text-to-SQL methods on four well recognized datasets, Spider~\citep{sprder2018} and Spider-Realistic~\citep{deng2021}. Spider is a large-scale cross-domain Text-to-SQL dataset, which contains 8659 instances in training split and 1034 instances in development split over 200 databases. Each instance is consisted of a natural language
% question on a specific database and its corresponding SQL query. In
% this paper, we use the development split Spider-dev for the purpose
% of evaluation as the test split is not released. Spider-Realistic
% is a more challenging variant of Spider. It selects a subset of 508
% examples from Spider-dev and manually revises the questions while
% keeping the SQL queries unchanged. For few-shot scenarios, we
% utilize the training split of Spider as the example candidates when
% testing with both Spider-dev and Spider-Realistic.



\paragraph{Main Result in Zero-shot Setting.}

\paragraph{Main Result in Few-shot Setting.}

\paragraph{Main Result in Fine-tuning Setting.}

\paragraph{Analysis I: Zero shot vs Few-shot.}


\paragraph{Analysis II: Zero shot / Few Shot vs Fine-Tuning.}


\paragraph{Analysis 2: }


\subsection{Supervised Fine-Tuning}

\subsubsection{Default Setting}


\begin{table*}[tbh]
\begin{center}
\scalebox{0.85}{
\begin{tabular}{ l c c c c}
\toprule
& Spider & BIRD & SPARC & WikiSQL \\

\bottomrule
\end{tabular}}
\end{center}
\caption{xx.}
\label{tab:xx}
\vspace{-2mm}
\end{table*}



\begin{table}[htbp]
    \centering
    \resizebox{0.9\linewidth}{!}
    {
    \begin{tabularx}{1.\textwidth}{c|c|cc|cc|cc|cc}
    \toprule
         \textbf{Dataset} & \textbf{SFT} & \multicolumn{2}{c}{\textbf{Spider}}  & \multicolumn{2}{c}{\textbf{BIRD}} & \multicolumn{2}{c}{\textbf{SPARC}} & \multicolumn{2}{c}{\textbf{WikiSQL}} \\ \hline
         \textbf{Metrics}& ~ & EX & EM & EX& EM & EX & EM & EX & EM \\ \hline
        \multirow{3}*{Baichuan-7b} 
        ~ & base  & 33.5 &  &  &  &  &  &  & \\
      ~ & qLora & 68.0 &  &  &  &  &  &  &  \\
      ~ & Lora  & 62.4 &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{Qwen7b} 
        ~ & base &  23.5 &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  & 66.2 &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{codellama7b-instruct} 
        ~ & base  &  &  &0.85  &  &  &  &  & \\
      ~ & qLora &  &  &  23.66 & &  &  &  &  \\
      ~ & Lora  &  &  &  22.29 &  &  &  &  &  \\ \hline  
        \multirow{3}*{chatglm3-6b} 
        ~ & base  &  &  & 0.00 &  &  &  &  & \\
      ~ & qLora &  &  & 13.89 &  &  &  &  &  \\
      ~ & Lora  &  &  & 15.58 &  &  &  &  &  \\ \hline
        \multirow{3}*{llama7b} 
        ~ & base  & 0.0  & 0.0 &  &  &  &  &  & \\
      ~ & qLora & 62.5 & 56.4 &  &  &  &  &  &  \\
      ~ & Lora  & 63.7 & 58.1 &  &  &  &  &  &  \\ \hline
        \multirow{3}*{baichuan2-13b} 
        ~ & base  & 39.2 & 15.5 & 3.52 & 0.07 &  &  &  & \\
      ~ & qLora &  68.8& 60.6 & 13.62 &3.72  &  &  &  &  \\
      ~ & Lora  & 65.9 & 60.7 & 17.60 & 4.50 &  &  &  &  \\ \hline
        \multirow{3}*{qwen14b} 
        ~ & base  & 57.3 & 35.9 & 13.10 & 0 &  &  &  & \\
      ~ & qLora & 73.6 & 66.5 & 19.88 & 5.93 &  &  &  &  \\
      ~ & Lora  & 70.1 & 66.8 & 22.56 & 6.39 &  &  &  &  \\ \hline
        \multirow{3}*{codellama13b-instruct} 
        ~ & base  &  &  & 8.93 &  &  &  &  & \\
      ~ & qLora &  &  & 29.34 &  &  &  &  &  \\
      ~ & Lora  &  &  & 29.40 &  &  &  &  &  \\ \hline
        \multirow{3}*{llama13b} 
        ~ & base  & 0.0 & 0.0 &  &  &  &  &  & \\
      ~ & qLora &  71.9& 64.0 &  &  &  &  &  &  \\
      ~ & Lora  & 71.1 & 63.2 &  &  &  &  &  &  \\ \hline
     \hline
    \end{tabularx}
    }
    \caption{The metrics of different models on four datasets with default setting}
    \label{tab:result_fix}
    \vspace{-5mm}
\end{table}


\subsubsection{Different Prompt Representation}
\begin{table}[h]
    \centering
    \resizebox{1.\linewidth}{!}
    {
    \begin{tabularx}{1.5\textwidth}{c|c|cc|cc|cc|cc|cc}
    \toprule
         \textbf{Prompt Representation} & \textbf{SFT} & \multicolumn{2}{c}{\textbf{Basic Prompt}}  & \multicolumn{2}{c}{\textbf{Text Representation}} & \multicolumn{2}{c}{\textbf{OpenAI Demostration}} & \multicolumn{2}{c}{\textbf{Code Representation}} & \multicolumn{2}{c}{\textbf{Alpaca SFT}}\\ \hline
         \textbf{Metrics}& ~ & EX & EM & EX& EM & EX & EM & EX & EM & EX & EM \\ \hline
        \multirow{3}*{Baichuan-7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{Qwen7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{codellama7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline  
        \multirow{3}*{chatglm3-6b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{llama7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{baichuan2-13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{qwen14b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{codellama13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{llama13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
     \hline
    \end{tabularx}
    }
    \caption{The metrics of different prompt representations on Spider datasets. }
    \label{tab:result_fix}
    \vspace{-5mm}
\end{table}


\subsubsection{Different Number of Prompt}
\begin{table}[h]
    \centering
    \resizebox{0.8\linewidth}{!}
    {
    \begin{tabularx}{1.\textwidth}{c|c|cc|cc|cc|cc|cc}
    \toprule
         \textbf{Number of Prompt} & \textbf{SFT} & \multicolumn{2}{c}{\textbf{Zero}}  & \multicolumn{2}{c}{\textbf{1}} & \multicolumn{2}{c}{\textbf{2}} & \multicolumn{2}{c}{\textbf{5}} & \multicolumn{2}{c}{\textbf{10}}\\ \hline
         \textbf{Metrics}& ~ & EX & EM & EX& EM & EX & EM & EX & EM & EX & EM \\ \hline
        \multirow{3}*{Baichuan-7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{Qwen7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{codellama7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline  
        \multirow{3}*{chatglm3-6b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{llama7b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{baichuan2-13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{qwen14b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{codellama13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
        \multirow{3}*{llama13b} 
        ~ & base  &  &  &  &  &  &  &  & \\
      ~ & qLora &  &  &  &  &  &  &  &  \\
      ~ & Lora  &  &  &  &  &  &  &  &  \\ \hline
     \hline
    \end{tabularx}
    }
    \caption{The metrics of different numbers of examples on Spider datasets. \Dqi{SFT performance comparison by varying the number of examples on Spider dataset.} }
    \label{tab:result_fix}
    \vspace{-5mm}
\end{table}


\subsubsection{RLHF}


\subsubsection{RL}


==> latex/preliminary.tex <==
\subsection{A Generalized Setup}
The input of text-to-SQL task is a natural language question $q$ and the database information $\db$. The output is the SQL $s$ corresponding to the question. The database $\db = \{S, K_p, K_f\}$ includes database schema $S$, primary keys $K_p$ and foreign keys $K_f$, where $S$ usually contains multiple tables $T_k: S = \{T_1, T_2, ...T_s...\}$. Each table $T_k$ has table name $N_k$,
column names $c_j$ and column data types $t_j$. Therefore, $T_k = \{N_k,(c_{k1}, t_{k1}),(c_{k2}, t_{k2})...\}$. Consider the queries may come from various database domains, we formulate the data into a set of triples $\mathcal{M}=\{(q_i, s_i, \db_i)\}$, with $i$ denoting the index of the query, the output and source database. 

%\textcolor{blue}{Given a natural language query $\mathcal{Q}$ and a database $\db = \{\mathcal{T}, \mathcal{C}\}$, the objective of Text-to-SQL task is to generate the corresponding SQL query $\mathcal{Y}$ w.r.t. $\mathcal{Q}$, where $\mathcal{T} = \{t_1, \cdots, t_n\}$ represents $n$ tables in $D$, and  .}

% Primary keys
% Kp uniquely identify rows of each table, and foreign keys Kf used to combine ("join") multiple tables


\subsection{Prompt-based and Fine-tuning Settings}
\label{sec:prompt_ft_setting}
Based on how LLMs are used for text-to-SQL generations, the problem settings can be categorized into three scenarios: zero-shot prompting, few shot prompting and fine-tuning. 

\paragraph{Zero-shot Prompting.} In zero-shot scenarios, no exemplar is provided and the main challenge is to represent the natural language question effectively. Formally, given an LLM parameterized by $\theta$, the question $q_i$ and the database $\db_i$, the objective is maximize the probability of generating the correct SQL $s_i$ from the LLM: 
%$\max_{\sigma} \mathbb{P}_{\theta}(s_i \vert \sigma(q_i, \db_i)),$
\begin{align}
\max_{\sigma} \mathbb{P}_{\theta}(s_i \vert \sigma(q_i, \db_i)),
\end{align}
where ${\Theta}$ and $\sigma(q_i, \db_i)$ \footnote{$\sigma(q_i, \db_i)$ technically denotes the information set generated by $q_i$ and $\db_i$.} denotes a representation of the target question $q_i$ by incorporating relevant information from $\db_i$. Following~\citet{gao2023texttosql}, we use 
the widely-used and effective \textit{Text Representation Prompt} (TRP) prompt formats in SQL question representations throughout the paper. Shown in \Cref{lst:trp}, TRP represents questions and schemas in natural language along with instructions, e.g., ``Given the table schemas, please write the queries to answer the questions.''. 

% we name the process of representing a natural language question with database information as \emph{question representation} and we use 
% the widely-used \textit{Text Representation Prompt} (TRP) prompt formats of question representations:

% Shown in \Cref{lst:trp}, it represents questions and schemas in natural language along with instructions, e.g., ``Given the table schemas, please write the queries to answer the questions.''. 


% \begin{itemize}[leftmargin=*]
%     \item Basic Prompt (BP). Illustrated in \Cref{lst:bp}, it is the prompt in a basic and straightforward form, which consists of table schemas,
%          a question prefixed by ``Q:'' and a response prefix ``A: SELECT'', without any specific instructions.
%     % \item Text Representation Prompt (TRP). Proposed by~\citep{enhancing} , it represents both schemas and questions in natural language. It also adds instruction at the very beginning of the prompt.
%     \item Text Representation Prompt (TRP). Shown in \Cref{lst:trp}, it represents questions and schemas in natural language along with instructions, e.g., ``Given the table schemas, please write the queries to answer the questions.''. 
    
%     % Compared with TRP, the instruction in R-TRP is specified with an explicit rule, e.g., ``Complete sqlite SQL query only and with no explanation''..
%     \item Code Representation Prompt (CRP). Illustraed in \Cref{lst:crp},  CRP directly
% presents ``CREAT TABLE'' SQLs, and prompts LLM with
% natural language question in comments. It stands out due to its ability to provide comprehensive information necessary for database creation, such as column types and keys~\citep{enhancing,openaiprompt}.
% %     \item Alpha fine-tuning Prompt (AFTP). It is the prompt designed for fine-tuning~\citep{alpaca}, which prompts LLMs to follow instruction and finish
% % task according to the input context in Markdown format.
% \end{itemize}

% The full examples of few-shot prompting in BP, TRP and CRP format can be found at \cref{lst:full_bp}, \cref{lst:full_trp} and \cref{lst:full_crp}, respectively in \cref{app:few_shot_example}.

The full examples of few-shot prompting in TRP format can be found at \cref{lst:full_trp} in \cref{app:few_shot_example}.


% \begin{lstlisting}[caption={Format of Basic Prompt.},label={lst:bp}]
% Table course, columns = [*,course_id,title,dept_name,credits]
% Table prereq, columns = [*,course_id,prereq_id]
% @
% \sethlcolor{humanpurple}  
% \hl{
% Q: 
% }
% @ Find the title of courses that have two prerequisites.
% @
% \sethlcolor{aigold}  
% \hl{
% A: 
% }
% @ SELECT T1.title FROM course AS T1 JOIN prereq AS T2 ON T1.course_id = T2.course_id GROUP BY T2.course_id HAVING count(*) = 2

% \end{lstlisting}


\begin{lstlisting}[caption={Format of Text Representation Prompt.},label={lst:trp}]
Given the following database schema,
Table course, columns = [*,course_id,title,dept_name,credits]
Table prereq, columns = [*,course_id,prereq_id]

@
\sethlcolor{humanpurple}  
\hl{
Please write queries to answer the questions:
}
@ 
Find the title of courses that have two prerequisites.
@
\sethlcolor{aigold}  
\hl{
Response: 
}
@ SELECT T1.title FROM course AS T1 JOIN prereq AS T2 ON T1.course_id = T2.course_id GROUP BY T2.course_id HAVING count(*) = 2.

\end{lstlisting}


% \begin{lstlisting}[caption={Format of Code Representation Prompt.},label={lst:crp}]
% Given the following SQL tables, your job is to write queries given a user's request.
    
%     CREATE TABLE courses (
%       course_id int,
%       title str,
%       dept_name str,
%       credits int,
%       PRIMARY KEY (course_id)
%     );
    
%     CREATE TABLE prereq (
%       course_id int,
%       prereq_id int,
%       PRIMARY KEY (course_id)
%     )
% @
% \sethlcolor{humanpurple}  
% \hl{
% Q: 
% }
% @ Find the title of courses that have two prerequisites.
% @
% \sethlcolor{aigold}  
% \hl{
% Response: 
% }
% @ SELECT T1.title FROM course AS T1 JOIN prereq AS T2 ON T1.course_id = T2.course_id GROUP BY T2.course_id HAVING count(*) = 2.

% \end{lstlisting}

% The main challenge is to represent the natural language question effectively, including incorporating relevant information such as the corresponding database schema~\citep{chang2023,dong2023c3}. 

% We define the process of representing natural language questions
% and relevant information as \textbf{query representation}.



\paragraph{Few-shot Prompting.} In few-shot scenarios, a few input–output exemplars are provided to prompt LLMs. The objective becomes 
$
\max_{\sigma} \mathbb{P}_{\theta}(s_i \vert \sigma(q_i, \mathcal{D}_i, \mathcal{M})), \quad \vert \mathcal{M} \vert =k
$
% \mathbb{P}_{\theta}(s_i \vert \sigma(q_i, \mathcal{D}_i, \mathcal{M})), \quad \vert \mathcal{M} \vert =k
Note that the database $\db_i$ is not necessarily included in exemplars of $\mathcal{M}$, which refers to the \emph{cross domain} text-to-SQL task. In addition to question representation, we also need to study the sensitivity to the exemplars -- for instance, varing the number or the selection strategy of few-shot exemplars can cause of change of the accuracy rate of LLMs~\citep{zhao2021calibrate,shi2023language}. 

Build on prior works, we summarize two popular strategies for selecting examplers:
\begin{itemize}[leftmargin=*]
    \item Random. This strategy randomly samples $k$ examplers from
the available candidates.
    \item Question similarity. Inspired by~\citep{liu-etal-2022-makes}, this strategy chooses $k$ examplers with the most similar questions. The similarity is measured by the cosine similarity between the encoded question pairs using a pretrained language model (LM).
\end{itemize}
In retrospect, we realize that there are more advanced strategies, such as generative query similarity used in DAIL-SQL~\citep{gao2023texttosql}. We conduct the analysis in xx. \siqiao{Add the analysis.}

\paragraph{Fine-tuning.} Prior studies~\citep{Sun2023SQLPaLMIL,gao2023texttosql} show that, although some popular LLMs, such as CodeX~\citep{chen2021evaluating} and ChatGPT~\citep{gpt3}, have shown successful results with ICL for text-to-SQL, they
still have a gap with the fine-tuned alternatives with median-sized LLMs. Specifically, the object of fine-tuning is minimize the empirical loss:
$\min_{\theta, \sigma} \mathcal{L}(s_i(\theta), \sigma(q_i, \db_i)),$
where $\mathcal{L}$ is the loss function to measure the difference between the generated SQL and the groundtruth. Note that, the fine-tuning covers two sub-tasks, including fine-tuning the LLM using supervised data in order to get the optimal $\theta$ 
, and searching for the optimal question representation $\sigma$.



